DNCs Require More Planning Steps

Many recent works use machine learning models to solve various complex algorithmic problems. However, these models attempt to reach a solution without considering the problem's required computational complexity, which can be detrimental to their ability to solve it correctly. In this work we investigate the effect of computational time and memory on generalization of implicit algorithmic solvers. To do so, we focus on the Differentiable Neural Computer (DNC), a general problem solver that also lets us reason directly about its usage of time and memory. In this work, we argue that the number of planning steps the model is allowed to take, which we call "planning budget", is a constraint that can cause the model to generalize poorly and hurt its ability to fully utilize its external memory. We evaluate our method on Graph Shortest Path, Convex Hull, Graph MinCut and Associative Recall, and show how the planning budget can drastically change the behavior of the learned algorithm, in terms of learned time complexity, training time, stability and generalization to inputs larger than those seen during training.

==> figures/mincut-extensions.tex <==
\begin{figure}[!htbp]
    \centering
    \begin{subfigure}{0.49\linewidth}
   \centering
   \includegraphics[width=\linewidth]{images/mincut/constant-mem-extension.png}
   \caption{Reweighted memory extension for model trained with $p(n)=10$, on MinCut.}
   \label{fig:mc-constant-mem-extend} 
\end{subfigure}
    \hfill
    \begin{subfigure}{0.49\linewidth}
   \centering
   \includegraphics[width=\linewidth]{images/mincut/linear-mem-extension.png}
   \caption{Reweighted memory extension for model trained with a $p(n)=\abs{E}$, on MinCut.}
   \label{fig:mc-linear-mem-extend}
\end{subfigure}
    \\[\baselineskip]
    \caption{
        \textbf{Reweighted Memory Extension on MinCut} - On this harder problem it appears that the models did not learn to utilize memory, as linear time budget might not be sufficient.
        }
    \label{fig:mincut-extensions}
\end{figure}

==> sections/theoretical.tex <==
\section{Discussion}
\label{sec-theory}
% - We want to analyze the impact of planning budget as a question of algorithm complexity, which is difficult to do for a neural network. The model could find an efficient representation of the data that allows it to, for example, query a graph's node as well as it's children in a single read operation (i.e. the memory cell value represents an efficient, aggregated piece of information about the input).

% - However it is clear that the amount of information the learned embedding space can contain is finite; in fact its implicit dimensionality is often much smaller than its embedding dimension \cite{ansuini2019intrinsic}.

% - This means that we can assume the embedding space allows the model an "efficiency factor" which is bounded and not too large, compared with a Turing Machine; i.e. its complexity can be 
% \todo[inline]{N: this is cute! interesting how can someone bound or even quantify this idea}
% - This means we can apply important results in complexity theory from which we know some problems are impossible to solve by a Turing machine in constant time.

% - This means the DNC could never solve them either, unless given a non-constant planning budget.

\subsection{Representation Spaces}
\label{sec-representation-spaces}
Similarly to \cite{neural_algorithmic_reasoning}, we can split the DNC's operation into two main parts: learning a representation space of the input \& output space, and learning to process these representations.
This representation is comprised of the embedding spaces the model utilizes: the learned memory embedding space $\mathcal{M}$ and the controller's state vector $h$, whose space we denote $\mathcal{H}\subset \R^{c}$. The model's goal for this joint representation space is to both accurately describe the input, in order for the result to be correct, and to allow modifications and processing during the operation of the learned algorithm.

We can now compare the operation of two DNC models, $A_1$ and $A_2$, whose planning budgets during training were $p_1 << p_2$.
Since its planning budget was smaller during training, model $A_1$ has two options: either find a faster algorithm to process the same representation space, or improve the representation efficiency of $\mathcal{M}\times\mathcal{H}$.
Due to the discussion in Section \ref{subsec-time-complexity}, we can assume that for large enough training inputs the first option is impossible, or at least very difficult. Thus the model is more likely to search for a more efficient representation.

However, and since the model learns to minimize the average loss over random instances of the problem, improving the efficiency of the embedding can be more easily achieved by finding more average-case, aggregate features in the data. This in turn encourages overfitting.



\todo[inline]{move thie example to appendices}
We can give an illustrative example for aggregate features the DNC model might overfit to, in the shortest path problem. Since we sample random graphs with some number of nodes and average degree, the maximum degree of nodes in the average path will not be much higher than the average degree we used to generate the graph. This means the model could overfit to efficiently represent nodes with degree up to some value $d$. When encountering larger graphs, even if the average degree is the same, since the lengths of the target paths increases so does the distribution of the max degree along that path gets shifted to higher values. This means that a representation such as the one described will fail to accurately describe the information needed to find these paths.
We can similarly describe other average case features, e.g. attributes of certain graph families that are more common than others when sampling random graphs.

\todo[inline]{we aren't testing specific aggregations, only the final symptom}
This explanation of the planning budget's impact mechanism is testable. If the model is able to learn a general algorithm even with a constant planning budget, we can expect the model to be able to generalize to larger inputs relatively well.
% However we must take care to give the model enough planning steps during this test. The learned algorithm could have some small time complexity, such that a small constant $p$ was sufficiently long for the training dataset's graph sizes. However for larger inputs, $p$ could simply not be enough time for the learned algorithm to complete.
% So we also run the model that learned with a constant $p$, but with a linearly scaling planning budget.
To test this hypothesis, we trained a DNC model with a constant planning budget $p=10$, on the Graph Shortest Path problem. The number of edges in the training data was $\abs{E}\leq 75$, and we tested the model on graphs with $\abs{E}$ from 5 to 250.
We ran the model once with $p=10$ as it was trained, and once with $p=\abs{E}$.
If the model learned a generic algorithm during its training, it should be able to generalize well to larger inputs.

We observe this to be false; instead, DNC models with a constant $p$ barely manage to generalize at all. Increasing the planning budget to a linear or even a quadratic function of the input size substantially improves the learned algorithms' generalization abilities. 
The experiment is fully described in \todo{reference!}.

\subsubsection{Memory efficiency}
\label{sec-memory-efficiency}
Another important effect of a small planning budget is a less efficient utilization of the memory address space, due to two effects.
\todo[inline]{fewer reads == less memory ops == the model is worse at doing these ops == when it has to do more, it will fail}
First, since the representations saved in each memory cell are forced to be more efficient, the model requires fewer reads or writes to retrieve the information it needs in most cases, allowing the model to rely less on memory operations themselves.
Second, since the controller's state representation space $\mathcal{H}$ is also forced to become more efficient, it could act as a "scratch pad" storage area where the controller stores intermediate values instead of saving them to memory.
This intermediate value gets accumulated over the run time of the algorithm, and the model learns to manage this accumulation for input sizes and planning budgets seen during training.
However when generalizing to larger inputs, the controller's state won't be able to accurately hold the larger amount of information that gets accumulated over a longer run time, also producing errors.
A more general algorithm would prefer to use the memory matrix to store intermediate values instead.

We can also test a trained DNC's memory efficiency by allowing it to use a larger memory matrix than seen during training.
If the model learned to efficiently use its memory address space, then extending the number of available cells should allow it to generalize to even larger input sizes.
In our experiments we observe that the DNC trained with constant $p$ performs much worse with an extended memory than a DNC trained with linear or even quadratic $p$, as seen in \todo{image here!}.
Further details for this experiment are described in \todo{reference!}



==> tables/convex-curriculum.tex <==
\begin{table}[!htbp]
    \centering
    \begin{tabular}{|c|c|}
    \hline
     Lesson & Number   \\
            & of Points \\
        \hline
        1 & (5,20)   \\
        2 & (10,20)  \\
        3 & (15,25)  \\
        4 & (20,35)  \\
        \hline
    \end{tabular}
    \caption{\textbf{Convex Hull Task curriculum}}
    \label{tab:mincut-results}
\end{table}
